Robust Image Ordinal Regression with Controllable Image Generation

Image ordinal regression has been mainly studied along the line of exploiting the order of categories. However, the issues of class imbalance and category overlap that are very common in ordinal regression were largely overlooked. As a result, the performance on minority categories is often unsatisfactory. In this paper, we propose a novel framework called CIG based on controllable image generation to directly tackle these two issues. Our main idea is to generate extra training samples with specific labels near category boundaries, and the sample generation is biased toward the less-represented categories. To achieve controllable image generation, we seek to separate structural and categorical information of images based on structural similarity, categorical similarity, and reconstruction constraints. We evaluate the effectiveness of our new CIG approach in three different image ordinal regression scenarios. The results demonstrate that CIG can be flexibly integrated with off-the-shelf image encoders or ordinal regression models to achieve improvement, and further, the improvement is more significant for minority categories.

==> sec/rebuttal.tex <==
\newcommand{\marked}[1]{\textcolor{red}{#1}}

\newcommand{\vspacex}{\vspace{-1.5ex}}

\textit{We really appreciate the consistent positive opinions from all the reviewers %and thank all of you for your time and effort in reviewing our manuscript and providing insightful comments. 
and their comments that help us further improve our work.
Our detailed responses are given below.}

\vspacex
\section{Response to Reviewer \#1}
% #But the difference is not so significant. And although the accuracy for minority categories are increased by generating image, the accuracy for major categories are sometimes decreased.
\noindent\textbf{Q1. Marginal overall improvement and performance decrease for majority categories.}
The performance improvement is substantial on Adience (i.e., +2.7\% in ACC and $-0.02$ in MAE), and we agree that the overall improvement is less impressive on the other two datasets, due to the extremely uneven sample distributions across the categories (Sec.~4.2). Note that such class imbalance could easily cause robustness issues, and it is necessary to evaluate category-level performance from a subgroup fairness perspective. Indeed, our results in Sec.~4.3 verify that the marginal overall improvement could correspond to remarkable robustness and fairness improvement in the presence of class imbalance. Hence, we state in the paper that ``the improvement is also crucial".

Since our fusion image generation process is biased toward minority categories, it is quite possible that the performance on majority categories might decrease. Yet, we find that this happens only occasionally and the decrease is much slighter than the improvement on minority ones. Also, note that minority categories often have greater application values in practice. Thus, we think the occasional and slight performance drop on majority categories is a tolerable price to pay.

%While we achieved significant improvement on the Adience dataset, the overall improvement on the other two datasets is limited. We attribute this to the fact that one majority category has a data size that exceeds two-thirds of the overall dataset, which in turn, tends to average out the results.  Furthermore, in the ordinal regression task, we found that the performance on minority categories is poor. Our goal was to improve the performance on minority categories, and we validated this improvement in section 4.3. Given that minority categories hold greater value in practical applications, our method is significant. Although there is a drop in performance in the larger categories, it is not significant and does not occur frequently. We believe that this cost is affordable.

% Our method has brought overall improvement, surpassing the previous SOTA method by 2\% in ACC and 0.02 in MAE, and surpassing the baseline, for example, by 7\% in ACC and 0.08 in MAE on the Adience dataset. Compared with the previous methods, the improvement brought by them is similar to ours. 
% Otherwise, we have achieved very competitive results on the majority categories on all three datasets. For example, as shown in Figs 1a\&1b in supplementary material, the overall majority categories results of our method are higher than the best results of the other two methods on both ACC (76.21\% vs 75.60\%) and MAE (0.305 vs 0.325) on the Adience dataset.



\noindent\textbf{Q2. Extra ablation study results and examples of generated images.} 
% We only show the results on Adience dataset, because the ablation experimental results on all three datasets are consistent. 
Thank you for your suggestion. We will provide more experimental results of ablation study and examples of fusion images in the Supplementary Material.

\noindent\textbf{Q3. Reproducibility.} 
We used three public datasets to validate our approach and described our experimental setup in detail in the paper. In addition, we will open-source our code on GitHub if the paper is accepted. With these, we hope our results will be reproducible with reasonable effort.

% We used three public datasets, which are accessible, and present the overall structure of the proposed method and each part in section 3.1. The formula of each loss function is described in detail in section 3.2. reviewers \#2,\#3,\#4,\#5 also agree that our method is reproducible. We will open our source code on GitHub if accepted.

\vspacex
\section{Response to Reviewer \#2}

\textbf{Q1. Using the accuracy metric to differentiate the majority and minority categories.} 
Indeed, we find that the two metrics, i.e., accuracy and the number of samples, identify quite similar categories. This implies that class imbalance is a major cause of robustness issues.
In addition, in this paper, we argue that category overlap could also cause robustness problems for image ordinal regression. We do find some example categories with moderate numbers of samples and degraded performance (e.g., cls2 on the Aesthetic dataset and cls6 on the Adience dataset). Their samples are susceptible to being misclassified into adjacent majority categories. We thus choose the accuracy metric to unify both issues. We appreciate the reviewer's sharp comment, and will clarify our thinking behind using the metric.


% In the ordinal regression task, there are some reasons that cause poor classification performance. Some categories have poor classification performance because they contain few data samples and are easily ignored during training. But when a category is adjacent to a majority category with a lot of data samples(e.g., cls2 in the Aesthetics dataset and cls6 in the Adience dataset), the data of these minority categories will be easily misclassified to the major categories, so we also call these kinds of categories minority categories. \ying{***still confuse why using accuracy not number***}
% In the ordinal regression task, there are two types of categories, associated with the data imbalance, which will cause the classification performance to decrease. The first is that the category itself only contains a few samples, and the second is the category close to the majority category (i.e., having lots of samples). Explaining the second, for example, cls2 (13\% adjacent to 29\%) in the Aesthetics dataset and cls6 (24\% adjacent to 66\%) in the Adience dataset. The samples of these categories will be attracted by the majority category, resulting in poor classification performance. Both of these two types of categories, which we define as minority, lead to low accuracy. If we employ the number of samples to define minority, the second type cannot be included.
% Indeed, we observed that categories with fewer samples tended to have poorer classification performance. Therefore, we regarded all categories with performance significantly lower than the average as minority categories, to highlight that our method significantly improves the performance of poorly-performing categories. We appreciate the reviewer's suggestion and will emphasize the inherent correlation between sample volume and classification performance in the paper.

% We observed that categories with fewer samples tended to have poorer classification performance. However, we also discovered that some categories with normal sample sizes had similarly poor classification performance. Our analysis revealed that the latter occurred when the categories were close to majority categories, making them susceptible to being misclassified as the labels of the adjacent majority categories. As both of these categories were caused by the data distribution, we categorized them as minority categories (i.e., poorly-performing categories) to highlight the significant improvements our method achieved. We appreciate the reviewer's suggestion and will emphasize the inherent correlation between classification performance and data distribution in the paper.


\noindent\textbf{Q2. Motivation and processing of the S-F module.}
% We observe that the expression of a category in an image is dominated by a small part of the region in the image. Thus, we regard the features in that region as categorical features. Other features, irrelevant to the category, are the structure of the object, and we call them structural features. This is why we divide features into two types. 
We observe that images in ordinal regression tasks often share quite a bit of common features and their labels are determined by a relatively small number of category-determining features. We call the latter kind of features {\it categorical information}, and propose to explicitly extract them for better classification accuracy (c.f.~our continued training). We then call the remaining features {\it structural information} and this concept is borrowed from structural similarity which refers to the perceived similarity between images. In this sense, structural information could also be viewed as complementary to categorical information.
%but a small number of detailed features ultimately determine the class. Furthermore, inspired by the structural similarity index measure (SSIM), we believe that SSIM reflects the overall features of the samples. In our task, we applied this idea and regarded structural features as complementary features outside of the category features and as common features among samples. Therefore, we separated features into category features and structural features.
%
The process of the S-F module is as follows. First, we input the features $F^{(4)}$ of the reference image and the main image into the S-F module, corresponding to $F_m^{(4)}$ and $F_r^{(4)}$ in Fig.~2. Then we extract the structural features of the main image and the categorical features of the reference image through the categorical and structural extractors, and concatenate them together as input to the generation network. We will further reorganize these contents later in Sec.~3.1 to make this part of the description more clear.

\noindent\textbf{Q3. Figure 2 should be clearer.}
$F_m^{(4)}$ and $F_r^{(4)}$ shown in the S-F module in the upper-left corner of Fig.~2 represent the fourth output $F^{(4)}$ of the main image and the reference image, respectively. We will improve the description of the related parts to make them more clear.

\vspacex
\section{Response to Reviewer \#3}

\textbf{Q1. Comparison with SMOTE.} 
We think our work is very different from the other oversampling methods such as SMOTE and the recent mix-up strategies. Note that SMOTE uses $k$-means to find adjacent samples for interpolation-based oversampling, and mix-up is a random combination of original images with mixed labels. In comparison, our method is controllable, i.e., generating images of specific labels near class boundaries. To achieve this, we seek to separate the structural and categorical information of images in a hidden latent space, and the fusion is performed in that space. Finally, our generation process is biased toward certain (minority) categories.

Thank you for your suggestions. We will incorporate the above discussion into the related work. 
% The traditional SMOTE uses K-means to find neighbors to generate samples by interpolation. In order to use SMOTE on the image dataset, we employ the idea of mixup to improve the SMOTE method. After performing, the experimental result shows that SMOTE brings improvement in ACC but also increases MAE a lot. We believe this phenomenon is due to the confusion of labels in ordinal regression by mixing images. Unlike natural image classification, categorical features cannot coexist in ordinal regression tasks, because the existence of next-level features will cause previous-level features to be masked. 
% The experimental result will be presented in the supplementary material if the paper is accepted.
% , and the result is shown below:

% \begin{table}[h]
%     \centering
%     % \begin{tabular}{m{1.4cm}<{\centering} m{1.4cm}<{\centering}m{3.5cm}<{\centering} }
%     \begin{tabular}{ccc}
%         \hline
%         Method & ACC (\%)$\uparrow$ & MAE$\downarrow$ \\
%         Vgg-SMOTE & 61.04 & 0.58 \\
%         PVT-SMOTE & xxx & xxx \\
%         \hline
%     \end{tabular}
%     \caption{SMOTE result on Adience} % 
%     \label{tab:minority}
% \end{table}



\vspacex
\section{Response to Reviewer \#4}

\textbf{Q1. Future work discussion.} 
% As you suggested, we will add some future work discussions if accepted. First, we can see from the training curve that the training is oscillating during the generation process, which indicates that there is a quality gap between the generated image and the original image. Thus, how to generate high-quality images is the next goal to explore. 
% Second, our method does not perform very well on abstract datasets (e.g., Aesthetics) because the category features of abstract images are expressed in the whole image(e.g., composition, light, and shadow). But our generation network requires overall structural similarity rather than content similarity. Therefore, it is very difficult to re-compose the original image. We hope that future methods can solve this problem.
Thank you for your suggestion. In future work, we plan to explore language-guided image generation in order to enhance and expand controllability.


%Firstly, we hope that the idea of improving the performance of backbones by data generation can be extended to other domains in future work, such as 3D medical imaging, video, and even natural language processing.
% we aim to extend our method to a broader range of fields, such as processing and augmenting CT and MRI data in medical imaging to address the issue of limited medical image samples.
%Additionally, we intend to incorporate multi-modal features into our image generator, such as introducing textual features to better optimize the image generation process.



\vspacex
\section{Response to Reviewer \#5}

\textbf{Q1. Explain the advantage of the proposed method over other methods.} 
The advantages of our method are illustrated in Fig.~1: We generate extra data near category boundaries to supplement less-represented categories, and this allows the model to better estimate the true classification boundaries from both the raw and generated data. We will add more discussion of the advantages of our method in Sec.~1. % 
% First, we did not modify the classification network, so our method can be transferred to any ordinal regression method, either jointly trained or used as a pre-trained model. Second, we expanded the data samples and alleviated the unrobustness problem due to data imbalance by generating images with self-supervised tasks. At the same time, we enhanced the feature extraction ability of the classification network through this jointly-training task.

\noindent\textbf{Q2. Examine the performance of the proposed framework on other datasets.} 
We have evaluated our approach on three datasets in this work. These three datasets span a wide range of image ordinal regression tasks. Therefore, we believe our results are representative and generalizable.  In future work, we will apply our method to more datasets to examine its performance and applicability.
% The three used datasets include abstract and concrete, medical images and daily images, which cover most of the scenarios in ordinal regression tasks, and reviewer \#2 also shows that our experiments are adequate in strengths(4). 
% The historical dataset is to evaluate the picture capture time and it is an abstract dataset and the samples are balanced. Therefore, we did not test our method on other additional datasets.

